The Athena X-ray Integral Field Unit: a consolidated design for the system requirement review of the preliminary definition phase

The Athena X-ray Integral Unit (X-IFU) is the high resolution X-ray spectrometer, studied since 2015 for flying in the mid-30s on the Athena space X-ray Observatory, a versatile observatory designed to address the Hot and Energetic Universe science theme, selected in November 2013 by the Survey Science Committee. Based on a large format array of Transition Edge Sensors (TES), it aims to provide spatially resolved X-ray spectroscopy, with a spectral resolution of 2.5 eV (up to 7 keV) over an hexagonal field of view of 5 arc minutes (equivalent diameter). The X-IFU entered its System Requirement Review (SRR) in June 2022, at about the same time when ESA called for an overall X-IFU redesign (including the X-IFU cryostat and the cooling chain), due to an unanticipated cost overrun of Athena. In this paper, after illustrating the breakthrough capabilities of the X-IFU, we describe the instrument as presented at its SRR, browsing through all the subsystems and associated requirements. We then show the instrument budgets, with a particular emphasis on the anticipated budgets of some of its key performance parameters. Finally we briefly discuss on the ongoing key technology demonstration activities, the calibration and the activities foreseen in the X-IFU Instrument Science Center, and touch on communication and outreach activities, the consortium organisation, and finally on the life cycle assessment of X-IFU aiming at minimising the environmental footprint, associated with the development of the instrument. Thanks to the studies conducted so far on X-IFU, it is expected that along the design-to-cost exercise requested by ESA, the X-IFU will maintain flagship capabilities in spatially resolved high resolution X-ray spectroscopy, enabling most of the original X-IFU related scientific objectives of the Athena mission to be retained. (abridged).

==> exp_ast_authors.tex <==
\author[1]{Didier Barret}
\author[2]{Vincent  Albouys}
\author[3]{Jan-Willem den Herder}
\author[4]{Luigi Piro}
\author[5]{Massimo Cappi}
\author[6]{Juhani Huovelin}
\author[7]{Richard Kelley}
\author[8]{J. Miguel Mas-Hesse}
\author[9]{Stéphane Paltani}
\author[10]{Gregor Rauw}
\author[11]{Agata Rozanska}
\author[12]{Jiri Svoboda}
\author[13]{Joern Wilms}
\author[14]{Noriko Yamasaki}
\author[9]{Marc Audard}
\author[7]{Simon Bandler}
\author[15]{Marco Barbera}
\author[16]{Xavier Barcons}
\author[9]{Enrico Bozzo}
\author[16]{Maria Teresa Ceballos}
\author[17]{Ivan Charles}
\author[3]{Elisa Costantini}
\author[13]{Thomas Dauser}
\author[18]{Anne Decourchelle}
\author[17]{Lionel Duband}
\author[17]{Jean-Marc Duval}
\author[19]{Fabrizio Fiore}
\author[20]{Flavio Gatti}
\author[21]{Andrea Goldwurm}
\author[3]{Roland den Hartog}
\author[22]{Brian Jackson}
\author[3]{Peter Jonker}
\author[7]{Caroline Kilbourne}
\author[6]{Seppo Korpela}
\author[4]{Claudio Macculi}
\author[23]{Mariano Mendez}
\author[24]{Kazuhisa Mitsuda}
\author[25]{Silvano Molendi}
\author[1]{François Pajot}
\author[1]{Etienne Pointecouteau}
\author[7]{Frederick Porter}
\author[18]{Gabriel W. Pratt}
\author[21]{Damien Prêle}
\author[1]{Laurent Ravera}
\author[26]{Kosuke Sato}
\author[27]{Joop Schaye}
\author[28]{Keisuke Shinozaki}
\author[29]{Konrad Skup}
\author[30]{Jan Soucek}
\author[31]{Tanguy Thibert}
\author[32]{Jacco Vink}
\author[1]{Natalie Webb}
\author[2]{Laurence Chaoul}
\author[2]{Desi Raulin}
\author[3]{Aurora Simionescu}
\author[33]{Jose Miguel Torrejon}
\author[18]{Fabio Acero}
\author[34]{Graziella Branduardi-Raymont}
\author[5]{Stefano Ettori}
\author[6]{Alexis Finoguenov}
\author[35]{Nicolas Grosso}
\author[3]{Jelle Kaastra}
\author[36]{Pasquale Mazzotta}
\author[37]{Jon Miller}
\author[8]{Giovanni  Miniutti}
\author[38]{Fabrizio Nicastro}
\author[39]{Salvatore Sciortino}
\author[14]{Hiroya Yamaguchi}
\author[1]{Sophie Beaumont}
\author[2]{Edoardo Cucchetti}
\author[4]{Matteo D'Andrea}
\author[40]{Megan Eckart}
\author[18]{Philippe Ferrando}
\author[1]{Elias Kammoun}
\author[4]{Simone Lotti}
\author[2]{Jean-Michel Mesnager}
\author[4]{Lorenzo Natalucci}
\author[2]{Philippe Peille}
\author[3]{Jelle de Plaa}
\author[21]{Florence Ardellier}
\author[41]{Andrea Argan}
\author[2]{Elise Bellouard}
\author[2]{Jérôme Carron}
\author[42]{Elisabetta Cavazzuti}
\author[25]{Mauro Fiorini}
\author[3]{Pourya Khosropanah}
\author[17]{Sylvain Martin}
\author[7]{James Perry}
\author[18]{Frederic Pinsard}
\author[2]{Alice Pradines}
\author[20]{Manuela Rigano}
\author[22]{Peter Roelfsema}
\author[2]{Denis Schwander}
\author[43]{Guido Torrioli}
\author[44]{Joel Ullom}
\author[45]{Isabel Vera}
\author[5]{Eduardo Medinaceli Villegas}
\author[11]{Monika Zuchniak}
\author[2]{Frank Brachet}
\author[39]{Ugo Lo Cicero}
\author[44]{William Doriese}
\author[44]{Malcom Durkin}
\author[5]{Valentina Fioretti}
\author[2]{Hervé Geoffray}
\author[31]{Lionel Jacques}
\author[13]{Christian Kirsch}
\author[7]{Stephen Smith}
\author[46]{Joseph Adams}
\author[2]{Emilie Gloaguen}
\author[3]{Ruud Hoogeveen}
\author[3]{Paul van der Hulst}
\author[47]{Mikko Kiviranta}
\author[22]{Jan van der Kuur}
\author[2]{Aurélien Ledot}
\author[3]{Bert-Joost van Leeuwen}
\author[3]{Dennis van Loon}
\author[2]{Bertrand Lyautey}
\author[1]{Yann Parot}
\author[46]{Kazuhiro Sakai}
\author[3]{Henk van Weers}
\author[3]{Shariefa Abdoelkariem}
\author[17]{Thomas Adam}
\author[35]{Christophe Adami}
\author[2]{Corinne Aicardi}
\author[3]{Hiroki Akamatsu}
\author[33]{Pablo Eleazar Merino Alonso}
\author[1]{Roberta Amato}
\author[2]{Jérôme André}
\author[5]{Matteo Angelinelli}
\author[45]{Manuel Anon-Cancela}
\author[18]{Shebli Anvar}
\author[45]{Ricardo Atienza}
\author[17]{Anthony Attard}
\author[5]{Natalia Auricchio}
\author[45]{Ana Balado}
\author[17]{Florian Bancel}
\author[20]{Lorenzo Ferrari Barusso}
\author[2]{Vivian Bernard}
\author[45]{Alicia Berrocal}
\author[21]{Sylvie Blin}
\author[48]{Donata Bonino}
\author[2]{François Bonnet}
\author[17]{Patrick Bonny}
\author[12]{Peter Boorman}
\author[18]{Charles Boreux}
\author[18]{Ayoub Bounab}
\author[2]{Martin Boutelier}
\author[7]{Kevin Boyce}
\author[4]{Daniele Brienza}
\author[3]{Marcel Bruijn}
\author[5]{Andrea Bulgarelli}
\author[2]{Simona Calarco}
\author[49]{Paul Callanan}
\author[1]{Thierry Camus}
\author[2]{Florent Canourgues}
\author[48]{Vito Capobianco}
\author[50]{Nicolas Cardiel}
\author[1]{Florent Castellani}
\author[7]{Oscar Cheatom}
\author[7]{James Chervenak}
\author[43]{Fabio Chiarello}
\author[1]{Nicolas Clerc}
\author[17]{Laurent Clerc}
\author[16]{Beatriz Cobo}
\author[1]{Odile Coeur-Joly}
\author[21]{Alexis Coleiro}
\author[21]{Stéphane Colonges}
\author[48]{Leonardo Corcione}
\author[1]{Mickael Coriat}
\author[17]{Alexandre Coynel}
\author[5]{Francesco Cuttaia}
\author[51]{Antonino D'Ai}
\author[39]{Fabio D'anca}
\author[5]{Mauro Dadina}
\author[2]{Christophe Daniel}
\author[7]{Natalie DeNigris}
\author[3]{Johannes Dercksen}
\author[7]{Michael DiPirro}
\author[18]{Eric Doumayrou}
\author[3]{Luc Dubbeldam}
\author[1]{Michel  Dupieux}
\author[1]{Simon Dupourqué}
\author[17]{Jean Louis Durand}
\author[9]{Dominique Eckert}
\author[45]{Valvanera Eiriz}
\author[17]{Eric Ercolani}
\author[2]{Christophe Etcheverry}
\author[7]{Fred Finkbeiner}
\author[4]{Mariateresa Fiocchi}
\author[2]{Hervé Fossecave}
\author[31]{Philippe Franssen}
\author[3]{Martin Frericks}
\author[21]{Stefano Gabici}
\author[2]{Florent Gant}
\author[3]{Jian-Rong Gao}
\author[25]{Fabio Gastaldello}
\author[9]{Ludovic Genolet}
\author[25]{Simona Ghizzardi}
\author[45]{Mª Angeles Alcacera Gil}
\author[43]{Elisa Giovannini}
\author[1]{Olivier Godet}
\author[45]{Javier Gomez-Elvira}
\author[21]{Manuel Gonzalez}
\author[2]{Raoul Gonzalez}
\author[3]{Luciano Gottardi}
\author[1]{Dolorès Granat}
\author[18]{Michel Gros}
\author[2]{Nicolas Guignard}
\author[3]{Paul Hieltjes}
\author[45]{Adolfo Jesus Hurtado}
\author[52]{Kent Irwin}
\author[1]{Christian Jacquey}
\author[53]{Agnieszka Janiuk}
\author[2]{Jean Jaubert}
\author[45]{Maria Jiménez}
\author[2]{Antoine Jolly}
\author[17]{Thierry Jourdan}
\author[2]{Sabine Julien}
\author[54]{Bartosz Kedziora}
\author[7]{Andrew Korb}
\author[13]{Ingo Kreykenbohm}
\author[13]{Ole König}
\author[55]{Mathieu Langer}
\author[2]{Philippe Laudet}
\author[18]{Philippe Laurent}
\author[4]{Monica Laurenza}
\author[21]{Jean Lesrel}
\author[48]{Sebastiano Ligori}
\author[13]{Maximilian Lorenz}
\author[4]{Alfredo Luminari}
\author[55]{Bruno Maffei}
\author[2]{Océane Maisonnave}
\author[2]{Lorenzo Marelli}
\author[2]{Didier Massonet}
\author[2]{Irwin Maussang}
\author[45]{Alejandro Gonzalo Melchor}
\author[18]{Isabelle Le Mer}
\author[13]{Lea Michalski}
\author[2]{Jean-Pierre Millerioux}
\author[51]{Teresa Mineo}
\author[4]{Gabriele Minervini}
\author[1]{Alexeï Molin}
\author[2]{David Monestes}
\author[56]{Nicola Montinaro}
\author[1]{Baptiste Mot}
\author[1]{David Murat}
\author[3]{Kenichiro Nagayoshi}
\author[10]{Yaël Nazé}
\author[1]{Loïc Noguès}
\author[21]{Damien Pailot}
\author[4]{Francesca Panessa}
\author[20]{Luigi Parodi}
\author[1]{Pascal Petit}
\author[38]{Enrico Piconcelli}
\author[51]{Ciro Pinto}
\author[45]{Jose Miguel Encinas Plaza}
\author[45]{David Poyatos}
\author[17]{Thomas Prouvé}
\author[7]{Andy Ptak}
\author[42]{Simonetta Puccetti}
\author[56]{Elena Puccio}
\author[1]{Pascale Ramon}
\author[45]{Manuel Reina}
\author[2]{Guillaume Rioland}
\author[18]{Louis Rodriguez}
\author[2]{Anton Roig}
\author[17]{Bertrand Rollet}
\author[5]{Mauro Roncarelli}
\author[1]{Gilles Roudil}
\author[29]{Tomasz Rudnicki}
\author[2]{Julien Sanisidro}
\author[15]{Luisa Sciortino}
\author[3]{Vitor Silva}
\author[9]{Michael Sordet}
\author[1]{Javier Soto-Aguilar}
\author[2]{Pierre Spizzi}
\author[35]{Christian Surace}
\author[45]{Miguel Fernández Sánchez}
\author[3]{Emanuele Taralli}
\author[31]{Guilhem Terrasa}
\author[21]{Régis Terrier}
\author[56]{Michela Todaro}
\author[4]{Pietro Ubertini}
\author[25]{Michela Uslenghi}
\author[3]{Jan Geralt Bij de Vaate}
\author[3]{Davide Vaccaro}
\author[39]{Salvatore Varisco}
\author[21]{Peggy Varnière}
\author[55]{Laurent  Vibert}
\author[45]{María Vidriales}
\author[5]{Fabrizio Villa}
\author[45]{Boris Martin Vodopivec}
\author[42]{Angela Volpe}
\author[3]{Cor de Vries}
\author[7]{Nicholas Wakeham}
\author[2]{Gavin Walmsley}
\author[3]{Michael Wise}
\author[3]{Martin de Wit}
\author[11]{Grzegorz Woźniak}
\affil[1]{Institut de Recherche en Astrophysique et Planétologie, Université de Toulouse, CNRS, UPS, CNES 9, Avenue du Colonel Roche, BP 44346, F-31028, Toulouse Cedex 4, France}
\affil[2]{Centre National d'Etudes Spatiales, Centre spatial de Toulouse, 18 avenue Edouard Belin, 31401 Toulouse Cedex 9, France}
\affil[3]{SRON, Netherlands Institute for Space Research, Niels Bohrweg 4, 2333 CA Leiden, The Netherlands}
\affil[4]{Istituto di Astrofisica e Planetologia Spaziali, Via Fosso del Cavaliere 100, 00133, Roma, Italy}
\affil[5]{INAF, Osservatorio di Astrofisica e Scienza dello Spazio, via Gobetti 93/3, 40129, Bologna, Italy }
\affil[6]{Department of Physics, Faculty of Science, P.O. Box 64 (Gustaf Hällströmin katu 2), FI-00014, University of Helsinki, Finland}
\affil[7]{NASA Goddard Space Flight Center, 8800 Greenbelt Rd, Greenbelt, MD 20771, United States}
\affil[8]{Centro de Astrobiología (CSIC-INTA), Dep. de Astrofísica, Unidad María de Maeztu, European Space Astronomy Centre (ESA-ESAC), Camino Bajo del Castillo s/n - Villafranca del Castillo, 28692 Villanueva de la Cañada, Madrid, Spain}
\affil[9]{Département d'Astronomie, Université de Genève, Chemin d’Ecogia 16, CH-1290 Versoix, Switzerland}
\affil[10]{Université de Liège, Institut d'Astrophysique et de Géophysique, Quartier Agora, Allée du 6 Août 19c, B-4000 Liège 1 (Sart-Tilman), Belgium}
\affil[11]{Centrum Astronomiczne im. Mikołaja Kopernika Polskiej Akademii Nauk, ul. Bartycka 18, 00-716 Warszawa, Poland}
\affil[12]{Astronomical Institute, Czech Academy of Sciences, Bocni II 1401/1, CZ-14100 Praha 4, Czech Republic}
\affil[13]{Astronomical Institute of the FAU, Erlangen Centre for Astroparticle Physics, University of Erlangen-Nüremberg, Sternwartstr. 7, 96049 Bamberg, Germany}
\affil[14]{Institute of Space and Astronautical Science (ISAS), 3-1-1 Yoshinodai, Chuo-ku, Sagamihara, 252-5210, Japan}
\affil[15]{Università degli Studi di Palermo, Dipartimento di Fisica e Chimica, Via Archirafi 36, 90123 Palermo, Italy and INAF/Osservatorio Astronomico di Palermo G.S.Vaiana, Piazza del Parlamento 1, 90134 Palermo, Italy}
\affil[16]{Instituto de Física de Cantabria (CSIC-UC) Edificio Juan Jordá, Avenida de los Castros, s/n - E-39005 Santander, Cantabria, Spain}
\affil[17]{Département des Systèmes Basses Températures, CEA-Grenoble, 17 avenue des Martyrs, 38054 Grenoble cedex 99, France}
\affil[18]{Département d'Astrophysique, UMR AIM, Orme des Merisiers, Bât 709, 91191 Gif sur Yvette , France}
\affil[19]{INAF-Osservatorio Astronomico di Trieste, via Tiepolo 11, Trieste 34143, Italy}
\affil[20]{Università di Genova, Dipartimento di Fisica, Via Dodecaneso 33, 16146, Genova, Italy}
\affil[21]{Université Paris Cité, CNRS, CEA, Astroparticule et Cosmologie (APC), F-75013 Paris, France}
\affil[22]{SRON Netherlands Institute for Space Research, Landleven 12, 9747 AD Groningen, The Netherlands}
\affil[23]{Rijksuniversiteit Groningen, Faculty of Science and Engineering, Landleven 12, 9747 AD Groningen, The Netherlands }
\affil[24]{ National Astronomical Observatory of Japan, 2-21-1 Osawa, Mitaka, Tokyo 181-8588, Japan}
\affil[25]{INAF - IASF Milano, Via Alfonso Corti 12, I-20133 Milano, Italy}
\affil[26]{Department of Physics, Saitama University, 255 Shimo-Okubo, Sakura-ku, Saitama, 338-8570, Japan}
\affil[27]{Leiden Observatory, Leiden University, PO Box 9513, NL-2300 RA Leiden, The Netherlands}
\affil[28]{Japan Aerospace Exploration Agency, Research Unit II (U2), Research and Development Directorate, 305-8505 2-1-1, Sengen, Tsukuba, Ibaraki, Japan}
\affil[29]{Centrum Badan Kosmicznych, Polish Academy of Science, Bartycka 18a, 00-716 Warszawa, Poland}
\affil[30]{Institute of Atmospheric Physics, Czech Academy of Science, Bocni II 1401, 14131 Praha 4, Czech Republic}
\affil[31]{Centre Spatial de Liège, Liège Science Park, Avenue du Pré-Aily, 4031 Angleur, Belgium}
\affil[32]{Anton Pannekoek Institute/GRAPPA, University of Amsterdam, PO Box 94249, 1090 GE Amsterdam, The Netherlands}
\affil[33]{Instituto de Fisica Aplicada a las Ciencias y las Tecnologias, Universidad de Alicante, Carretera de San Vicente del Raspeig s/n, 03090 San Vicente del Raspeig, Alicante, Spain}
\affil[34]{Mullard Space Science Laboratory of University College London, Holmbury House, Holmbury St Mary, Dorking, Surrey, RH5 6NT, United Kingdom}
\affil[35]{LAM - Laboratoire d’Astrophysique de Marseille, Pôle de l’Étoile Site de Château-Gombert, 38, rue Frédéric Joliot-Curie 13388 Marseille cedex 13 FRANCE}
\affil[36]{Dipartimento di Fisica, Universita di Roma Tor Vergata, Via Della Ricerca Scientifica 1, I-00133, Roma, Italy}
\affil[37]{University of Michigan Department of Astronomy, 1085 South University Avenue, 323 West Hall, Ann Arbor, MI 48109-1107, United States }
\affil[38]{INAF - Osservatorio Astronomico di Roma, Via Frascati, 33, 00040, Monte Porzio Catone, Rome, Italy}
\affil[39]{INAF/Osservatorio Astronomico di Palermo G.S.Vaiana, Piazza del Parlamento 1, 90134 Palermo, Italy}
\affil[40]{Lawrence Livermore National Laboratory, 7000 East Avenue, L-509, Livermore CA 94550, United States}
\affil[41]{INAF Headquarter, Viale del Parco Mellini 84, 00136 Rome, Italy}
\affil[42]{Agenzia Spaziale Italiana, Unita' di Ricerca Scientifica, Via del Politecnico snc, 00133 Roma, Italia}
\affil[43]{Istituto di Fotonica et Nanotecnologie - Consiglio Nazionale Ricerche, Via Cineto Romano 42, 00156 Roma, Italia}
\affil[44]{National Institute of Standards and Technology, 325 Broadway, Boulder, CO 80305-3328, United States}
\affil[45]{INTA, Crtra de Ajalvir km 4, 28850, Torrejon de Ardoz, Madrid, Spain}
\affil[46]{University of Maryland Baltimore County, 1000 Hilltop Circle, Baltimore, MD 21250, United States}
\affil[47]{VTT, Tietotie 3, FIN-02150 Espoo, Finland}
\affil[48]{INAF - Osservatorio Astrofisico di Torino, Via Osservatorio 20, 10025 Pino Torinese, TO, Italy}
\affil[49]{University College Cork, College Rd, Cork, Ireland}
\affil[50]{Departamento de Física de la Tierra y Astrofísica, Facultad de Ciencias Físicas, Universidad Complutense de Madrid, Ciudad Universitaria, 28040-Madrid, Spain}
\affil[51]{IASF-Palermo, via Ugo La Malfa 153, 90146 Palermo}
\affil[52]{Stanford University, Stanford, California 94305, United States}
\affil[53]{Center for Theoretical Physics, Polish Academy of Sciences, Al. Lotnikow 32/46, 02-668 Warsaw, Poland}
\affil[54]{Astronika, ul. Bartycka 18, Office no. 33, 00-716 Warszawa, Poland}
\affil[55]{Institut d'Astrophysique Spatiale, Bât. 120-1, Université Paris Saclay, 91405, Orsay, France}
\affil[56]{Università degli Studi di Palermo, Dipartimento di Fisica e Chimica, Via Archirafi, 36, 90123, Palermo, Italy}

